G2L: A Geometric Approach for Generating Pseudo-labels that Improve Transfer Learning

Transfer learning is a deep-learning technique that ameliorates the problem of learning when human-annotated labels are expensive and limited. In place of such labels, it uses instead the previously trained weights from a well-chosen source model as the initial weights for the training of a base model for a new target dataset. We demonstrate a novel but general technique for automatically creating such source models. We generate pseudo-labels according to an efficient and extensible algorithm that is based on a classical result from the geometry of high dimensions, the Cayley-Menger determinant. This G2L (``geometry to label'') method incrementally builds up pseudo-labels using a greedy computation of hypervolume content. We demonstrate that the method is tunable with respect to expected accuracy, which can be forecast by an information-theoretic measure of dataset similarity (divergence) between source and target. The results of 280 experiments show that this mechanical technique generates base models that have similar or better transferability compared to a baseline of models trained on extensively human-annotated ImageNet1K labels, yielding an overall error decrease of 0.43\%, and an error decrease in 4 out of 5 divergent datasets tested.

==> labeling.tex <==
% incorporated into previous section

\label{sec:labeling}
% Generating rich pseudo-labels from models trained on distributionally similar data involves a trade off between an expressive, long label, and a generalizable, short label. Longer labels carry more information about similarity between previous models and the target image, and differences between the previously trained models could be critical for adequately labeling new examples. For example, an incoming set of data including pictures of household objects might be well described by combining the labels of “tool, fabric, furniture.” 

% However, domains that possess substantial differences from previous data might be better defined by the magnitude and direction of such a difference. For example, a ``flower'' dataset would share some features with ``plant,'' but it is perhaps better defined by statements such as ``flowers are very unlike furniture''.  In other, ambiguous cases, negative features may be necessary to distinguish between overlapping cases: a suit of armor might have similarities with the body shapes of people but could be contrasted with these categories by its dissimilarity with ``sport,'' a category otherwise close to ``person.''

% To label an image, we encode its relative positions with respect to some subset of the known labeled datasets. To better explain the technique, we will use ImageNet1K to source images and ground truth labels. ImageNet1K has 1,000 labels; the number of images/label is almost uniform; but the labels broadly fall under a few broad categories.
% For example, about 446 out of 1,000 labels ($\sim$ 45\%) belong to animals, while the other top categories are vehicle (5.2\%), food (2.2\%), musical instrument (2.1\%) and garment (2.1\%). The distribution of the number of labels for different categories, unlike the elephant, has a very long tail.

